Search for pair production of massive particles decaying into three quarks with the ATLAS detector in sqrt(s) = 7 TeV pp collisions at the LHC

A search is conducted for hadronic three-body decays of a new massive coloured particle in sqrt(s) = 7 TeV pp collisions at the LHC using an integrated luminosity of 4.6/fb collected by the ATLAS detector. Supersymmetric gluino pair production in the context of a model with R-parity violation is used as a benchmark scenario. The analysis is divided into two search channels, each optimised separately for their sensitivity to high-mass and low-mass gluino production. The first search channel uses a stringent selection on the transverse momentum of the six leading jets and is performed as a counting experiment. The second search channel focuses on low-mass gluinos produced with a large boost. Large-radius jets are selected and the invariant mass of each of the two leading jets is used as a discriminant between the signal and the background. The results are found to be consistent with Standard Model expectations and limits are set on the allowed gluino mass.

==> tools.tex <==

\RequirePackage{xspace}

%%% Event generator stuff
\newcommand{\Herwig}    {\texttt{Herwig}\xspace}
\newcommand{\herwigpp}  {\texttt{Herwig}++\xspace}
\newcommand{\Herwigpp}  {\herwigpp}
\newcommand{\geant}     {\texttt{GEANT}4\xspace}
\newcommand{\jimmy}     {\texttt{Jimmy}\xspace}
\newcommand{\Alpgen}    {\texttt{Alpgen}\xspace}
\newcommand{\Sherpa}    {\texttt{Sherpa}\xspace}
\newcommand{\Comphep}   {\texttt{CompHep}\xspace}
\newcommand{\Madgraph}  {\texttt{MadGraph}\xspace}
\newcommand{\Pythia}    {\texttt{PYTHIA}\xspace}
\newcommand{\Powheg}    {\texttt{POWHEG}\xspace}
\newcommand{\PowPythia} {\texttt{POWHEG}+\Pythia}
\newcommand{\Perugia}   {\texttt{Perugia}\xspace}
\newcommand{\Prospino}  {\texttt{Prospino}\xspace}
\newcommand{\Mcatnlo}   {\texttt{MC@NLO}\xspace}
\newcommand{\Acermc}    {\texttt{ACERMC}\xspace}
\newcommand{\PythiaP}   {\Pythia (\Perugia 2010)\xspace}
\newcommand{\ntilde}    {{\~ n}}
\newcommand{\LO}        {\ensuremath{\mathrm{LO}}\xspace}
\newcommand{\NLO}       {\ensuremath{\mathrm{NLO}}\xspace}
\newcommand{\NLL}       {\ensuremath{\mathrm{NLL}}\xspace}
\newcommand{\NNLO}      {\ensuremath{\mathrm{N}}\NLO\xspace}
\newcommand{\nLO}       {\nbar \LO\xspace}
\newcommand{\nNLO}      {\nbar \NLO\xspace}
\newcommand{\nnNLO}     {\nbar \nbar \NLO\xspace}
\newcommand{\nnLO}      {\nbar \nbar \LO\xspace}
\newcommand{\nNNLO}     {\nbar \NNLO\xspace}
\newcommand{\muF}       {\ensuremath{\mu_\textsc{f}}\xspace}
\newcommand{\muR}       {\ensuremath{\mu_\textsc{r}}\xspace}
\newcommand{\LS}        {\ensuremath{\mathrm{LS}}\xspace}
\newcommand{\nlojet}    {\textsc{NLOJet}\texttt{++}\xspace}
\newcommand{\TwoToTwo}  {\ensuremath{2\ra2}\xspace}

\newcommand{\SoverB}    {\ensuremath{S/B}\xspace}

%%% Energy
\newcommand{\fourfgev}  {\ensuremath{450~\mathrm{GeV}}\xspace}
\newcommand{\ninehgev}  {\ensuremath{900~\mathrm{GeV}}\xspace}
\newcommand{\seventev}  {\ensuremath{7~\mathrm{TeV}}\xspace}
\newcommand{\sqsfourt}  {\ensuremath{\sqrt{s} = 14~\mathrm{TeV}}\xspace}
\newcommand{\sqsTev}    {\ensuremath{1.96~\mathrm{TeV}}\xspace}
\newcommand{\threehtev} {\ensuremath{3.5~\mathrm{TeV}}\xspace}
\newcommand{\sqsnineh}  {\ensuremath{\sqrt{s} = \ninehgev}\xspace}
\newcommand{\sqsseven}  {\ensuremath{\sqrt{s} = \seventev}\xspace}
\newcommand{\bunchSp}   {\ensuremath{\tau_{\rm bunch}}\xspace}

\newcommand{\inwork}{{\bf This figure is still WORK IN PROGRESS.}}

\newcommand{\antikt}{anti-$k_{t}$}
\newcommand{\Antikt}{Anti-$k_{t}$}
\newcommand{\asym}{\ensuremath{\mathcal{A}}}
\newcommand{\Fastjet} {{\sc FastJet}\xspace}

%%% Luminosity
\newcommand{\invpb}     {~\ensuremath{{\rm pb}^{-1}}\xspace}
\newcommand{\invnb}     {~\ensuremath{{\rm nb}^{-1}}\xspace}
\newcommand{\invfb}     {~\ensuremath{{\rm fb}^{-1}}\xspace}
\newcommand{\invmub}    {~\ensuremath{\mu{\rm b}^{-1}}\xspace}
\newcommand{\cmSqSec}   {cm\ensuremath{^{-2}}s\ensuremath{^{-1}}\xspace}
\newcommand{\lumi}      {\ensuremath{\mathcal L}\xspace}
\newcommand{\calL}      {\lumi}
\newcommand{\dldz}      {\ensuremath{d\lumi/dz}\xspace}
\newcommand{\lofz}      {\ensuremath{{\mathcal L}(z)}\xspace}
\newcommand{\sigyofz}   {\ensuremath{\sigma_y(z)}\xspace}
\newcommand{\Lsp}       {\ensuremath{{\mathcal L}_{sp}}\xspace}
\newcommand{\StoB}      {\ensuremath{S/B}\xspace}
\newcommand{\pileup}    {pile-up\xspace}
\newcommand{\Pileup}    {Pile-up\xspace}

%
\newcommand{\JES}   {{\rm JES}}
\newcommand{\JMS}   {{\rm JMS}}
\newcommand{\EMJES} {{\rm EM+JES}}
\newcommand{\GCWJES}{{\rm GCW+JES}}
\newcommand{\LCWJES}{{\rm LCW+JES}}
\newcommand{\EM}    {{\rm EM}}
\newcommand{\GCW}   {{\rm GCW}}
\newcommand{\LCW}   {{\rm LCW}}
%
\newcommand{\GSL}   {{\rm GSL}}
\newcommand{\GS}    {{\rm GS}}

\newcommand{\MTF}   {{\rm MTF}}
\newcommand{\MPF}   {{\rm MPF}}
\newcommand{\Etmiss}   {\ensuremath{{E}_{\mathrm{T}}^{\mathrm{miss}}}}
\newcommand{\vecEtmiss}{\ensuremath{\vec{E}_{\mathrm{T}}^{\mathrm{miss}}}}

\newcommand{\EoverP}    {\ensuremath{E/p}}
\newcommand{\Etrue}     {\ensuremath{E^{\rm truth}}}
\newcommand{\Etruth}    {\ensuremath{E^{\rm truth}}}
\newcommand{\Ecalo}     {\ensuremath{E^{\rm jet}}}
\newcommand{\EcaloEM}   {\ensuremath{E^{\rm jet}_\EM}}
\newcommand{\Response}  {\ensuremath{\mathcal{R}}} 
\newcommand{\Rcalo}     {\ensuremath{\Response^{\rm jet}}} 
\newcommand{\RcaloM}    {\ensuremath{\Response^{\rm jet}_{M}}} 
\newcommand{\RcaloEM}   {\ensuremath{\Rcalo_\EM}}
\newcommand{\RMPF}      {\ensuremath{\Response_\MPF}}
\newcommand{\EcaloCALIB}{\ensuremath{E^{\rm jet}}}
\newcommand{\RcaloCALIB}{\ensuremath{\mathcal{R}^{\rm jet}}}

\newcommand{\EcaloEMJES} {\ensuremath{E^{\rm jet}_\EMJES}}
\newcommand{\RcaloEMJES} {\ensuremath{\mathcal{R}^{\rm jet}_\EMJES}}
\newcommand{\EcaloGCWJES}{\ensuremath{E^{\rm jet}_\GCWJES}}
\newcommand{\RcaloGCWJES}{\ensuremath{\mathcal{R}^{\rm jet}_\GCWJES}}
\newcommand{\EcaloLCWJES}{\ensuremath{E^{\rm jet}_\LCWJES}}
\newcommand{\RcaloLCWJES}{\ensuremath{\mathcal{R}^{\rm jet}^\LCWJES}}
\newcommand{\Rtrack}     {\ensuremath{\mathcal{R}^{\rm track  \; jet}}}

\newcommand{\rtrk}             {\ensuremath{r_{\rm trk}}\xspace}
\newcommand{\Rtrk}             {\ensuremath{R_{\rm trk}}\xspace}
\newcommand{\rtrackjet}        {\ensuremath{r^{\rm calo / track \; jet}}}
\newcommand{\rtrackjetiso}     {\ensuremath{\rtrackjet_{\rm iso}}}
\newcommand{\rtrackjetnoniso}  {\ensuremath{\rtrackjet_{\rm non-iso}}}
\newcommand{\rtrackjetisoratio}{\ensuremath{\rtrackjet_{\rm non-iso/iso}}}

\newcommand{\Rmin}       {\ensuremath{R_{\rm min}}}
\newcommand{\DeltaR}     {\ensuremath{\Delta R}}
\newcommand{\DetaDphi}   {\ensuremath{\sqrt{(\Delta \eta)^{2} + (\Delta\phi)^{2}}}\xspace}
\newcommand{\DyDphi}     {\ensuremath{\sqrt{(\Delta y)^{2} + (\Delta\phi)^{2}}}\xspace}
\newcommand{\DeltaRdef}  {\ensuremath{\DeltaR = \DetaDphi}\xspace}
\newcommand{\DeltaRydef} {\ensuremath{\DeltaR = \DyDphi}\xspace}
\newcommand{\DeltaRtrk}  {\ensuremath{\Delta R({\rm trk}_1,{\rm trk}_2)}}

\newcommand{\njet}      {\ensuremath{N_{\rm jet}}\xspace}
\newcommand{\Njet}      {\njet}
\newcommand{\JVF}       {\ensuremath{JVF}\xspace}


\newcommand{\etaDet}{\ensuremath{\eta_{\rm det}}}
%
\newcommand{\etatrk}{\ensuremath{\eta^{\rm track}}}

\newcommand{\etaRange}[2]{\ensuremath{{#1}\leq|\eta|<{#2}}}
\newcommand{\AetaRange}[1]{\ensuremath{|\eta|<{#1}}}

\newcommand{\gammajet}{\ensuremath{\gamma}\mbox{-}{\rm jet}}
\newcommand{\deltaphijetgamma}{\ensuremath{\Delta \phi_{{\rm jet}\mbox{-}\ensuremath{\gamma}}}}


\def\ltap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$<$}}
\def\gtap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$>$}}


\newcommand{\insitu}{{\textit{in situ}}\xspace}
\newcommand{\Insitu}{{\textit{In situ}}\xspace}
\newcommand{\pp}{\ensuremath{pp}\xspace}

\newcommand{\etjet}  {\ensuremath{\et^{\mathrm{jet}}}}
\newcommand{\ptavg}  {\ensuremath{\pt^\mathrm{avg}}}
\newcommand{\ptjet}  {\ensuremath{\pt^\mathrm{jet}}}
\newcommand{\ptRecoil}{\ensuremath{\pt^\mathrm{Recoil}}}
\newcommand{\ptLeading}{\ensuremath{\pt^\mathrm{Leading}}}
\newcommand{\ptjetEM}{\ensuremath{p_{\rm T, \EM}^\mathrm{jet}}}
\newcommand{\pthat}  {\ensuremath{\hat{p}_{\rm T}}}
\newcommand{\ptprobe}{\ensuremath{\pt^{\mathrm{probe}}}}
\newcommand{\ptref}  {\ensuremath{\pt^{\mathrm{ref}}}}
%
\newcommand{\ptRange}[2]{\ensuremath{{#1} \leq \ptjet<{#2} \GeV}}
\newcommand{\pttrue}  {\ensuremath{\pt^\mathrm{truth}}}
\newcommand{\pttruth} {\ensuremath{\pt^{\mathrm{truth}}}}
\newcommand{\pttrk}   {\ensuremath{\pt^{\mathrm{track}}}} 
\newcommand{\ptrk}    {\ensuremath{p^{\mathrm{track}}}} 
\newcommand{\pTtrkjet}{\ensuremath{p^{\mathrm{track \; jet}}_{\rm T}}}
\newcommand{\ntrk}    {\ensuremath{n_{\rm track}}} 

\newcommand{\sumPt}     {\ensuremath{\sum \vec{p}_{ \rm T}}}
\newcommand{\sumPtTr}   {\ensuremath{|\sum \vec{p}_{\rm T}^{\rm  track}|}}
\newcommand{\sumPtTrk}  {\ensuremath{\sum\pt^{\rm \ track}}\xspace}

\newcommand{\ptf}{\ensuremath{\pt^{\rm f}}}
\newcommand{\ptc}{\ensuremath{\pt^{\rm c}}}
\newcommand{\ptl}{\ensuremath{\pt^{\rm left}}}
\newcommand{\ptr}{\ensuremath{\pt^{\rm right}}}

\newcommand{\rapjet}{\ensuremath{y}}
\newcommand{\etajet}{\ensuremath{\eta}}
\newcommand{\phijet}{\ensuremath{\phi}}

\newcommand{\radlength}{\ensuremath{X_0}}


\newcommand{\topo} {topo-clust\-er}
\newcommand{\Topo} {Topo-clust\-er}
\newcommand{\topos}{topo-clust\-ers}
\newcommand{\Topos}{Topo-clust\-ers}

\newcommand{\central}{$0.3$ \ensuremath{\leq |\eta| < } $0.8$}
\newcommand{\ecap}   {$2.1$ \ensuremath{\leq |\eta| < } $2.8$}
\newcommand{\forward}{$3.6$ \ensuremath{\leq |\eta| < } $4.5$}

\newcommand{\Npv}{\ensuremath{N_{{\rm PV}}}}
\newcommand{\Nref}{\ensuremath{\Npv^{\rm ref}}}
\newcommand{\Navg}{\ensuremath{\langle \Npv \rangle}}

\newcommand{\ATLAS}   {ATLAS}
\newcommand{\Lone}    {\texttt{L1}}
\newcommand{\HLT}     {\texttt{HLT}}
\newcommand{\ID}      {\texttt{ID}}
\newcommand{\Pixel}   {\texttt{Pixel}}
\newcommand{\SCT}     {\texttt{SCT}}
\newcommand{\TRT}     {\texttt{TRT}}

\newcommand{\LHC}    {LHC}
\newcommand{\EMB}    {\texttt{EMB}}
\newcommand{\EME}    {\texttt{EME}}
\newcommand{\EMEC}   {\texttt{EMEC}}
\newcommand{\FCAL}   {\texttt{FCAL}}
\newcommand{\Cryo}   {\texttt{Cryo}}
\newcommand{\Gap}    {\texttt{Gap}}
\newcommand{\Scint}  {\texttt{Scint}}
\newcommand{\HEC}    {\texttt{HEC}}
\newcommand{\LAr}    {\texttt{LAr}}
\newcommand{\FCal}   {\texttt{FCal}}
\newcommand{\Tile}   {\texttt{Tile}}
\newcommand{\TileExt}{\texttt{TileExt}}
\newcommand{\TileBar}{\texttt{TileBar}}
\newcommand{\MBTS}   {\texttt{MBTS}}
\newcommand{\Presampler}   {\texttt{Presampler}}

%
\newcommand{\width}   {{\rm width}}

\newcommand{\ftile}{\ensuremath{f_{\Tile 0}}}
\newcommand{\fem}  {\ensuremath{f_{\LAr 3}}}
\newcommand{\fpres}{\ensuremath{f_{\rm PS}}}
\newcommand{\fhec} {\ensuremath{f_{\HEC 0}}}
\newcommand{\ffcal}{\ensuremath{f_{\FCal 1}}}


\newcommand{\btag   }{{\ensuremath{b}\mbox{\rm-tagging}}}
\newcommand{\btagged}{{\ensuremath{b}\mbox{\rm-tagged}}}
\newcommand{\bquark }{{\ensuremath{b}\mbox{\rm-quark}}}
\newcommand{\bquarks}{{\ensuremath{b}\mbox{\rm-quarks}}}
\newcommand{\Zbb}     {\ensuremath{Z\ra\bbbar}\xspace}
\newcommand{\tWb}     {\ensuremath{t \ra Wb}\xspace}
\newcommand{\Wqqbar}  {\ensuremath{W \ra \qqbar}\xspace}
\newcommand{\enu}       {\ensuremath{e\nu}\xspace}  
\newcommand{\Zmumu}     {\ensuremath{Z\ra\mumu}\xspace}
\newcommand{\Wlnu}      {\ensuremath{W\ra \lnu}\xspace}
\newcommand{\Wenu}      {\ensuremath{W\ra \enu}\xspace}
\newcommand{\munu}      {\ensuremath{\mu\nu}\xspace}
\newcommand{\Wmunu}     {\ensuremath{W\ra\munu}\xspace}
%
\newcommand{\bjet}{{\ensuremath{b}\mbox{-}{\rm jet}}}
\newcommand{\bjets}{{\ensuremath{b}\mbox{\rm-jets}}}
%

%
% User-defined latex commands for SUBSTRUCTURE
%

% Jet mass related
\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}     {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}  {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}      {\mjet}
\newcommand{\massjet}   {\mjet}
\newcommand{\mThresh}   {\ensuremath{M_{\rm threshold}}\xspace}
\newcommand{\mjetAvg}   {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}{\ensuremath{m^{\rm track \; jet}}\xspace}

\newcommand{\Wmass}     {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}    {\ensuremath{m^{\Wboson}_{T}}\xspace}
\newcommand{\topmass}   {\ensuremath{m_{\rm top}}\xspace}
\newcommand{\massZprime}{\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\akt}       {\antikt\xspace}
\newcommand{\Akt}       {\Antikt\xspace}
\newcommand{\AKT}       {\akt}
\newcommand{\AKTFat}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTPrune}  {\antikt, \ensuremath{R=1.0} (pruned)\xspace}
\newcommand{\AKTFilt}   {\antikt, \ensuremath{R=1.0} (filtered)\xspace}
\newcommand{\KTSix}     {\ensuremath{k_{t}}, \ensuremath{R=0.6}\xspace}
\newcommand{\kt}        {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}        {Cambridge-Aachen\xspace}
\newcommand{\CamKt}     {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}     {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}     {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}   {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}    {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}   {SISCone}
\newcommand{\SISConeSiz}{\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}     {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}    {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}    {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\Rij}       {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}      {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}   {\ensuremath{\frac{\DRij^2}{R^2}}\xspace}
\newcommand{\diB}       {\ensuremath{d_{iB}}\xspace}
\newcommand{\Rfilt}     {\ensuremath{R_{\rm filt}}\xspace}
\newcommand{\jone}      {\ensuremath{J_{1}}\xspace}
\newcommand{\jtwo}      {\ensuremath{J_{2}}\xspace}
\newcommand{\sjone}     {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}     {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}  {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}  {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\mjone}     {\ensuremath{m^{\jone}}\xspace}
\newcommand{\mjtwo}     {\ensuremath{m^{\jtwo}}\xspace}
\newcommand{\ptsubjone} {\ensuremath{p_{T}^{\sjone}}\xspace}
\newcommand{\ptsubjtwo} {\ensuremath{p_{T}^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}  {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets} {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\pti}       {\ensuremath{p_{{\rm T}i}}\xspace}
\newcommand{\ptj}       {\ensuremath{p_{Tj}}\xspace}
\newcommand{\ycut}      {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}      {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}      {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}     {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}    {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}      {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}      {\ensuremath{z_{\rm cut}}\xspace}
\renewcommand{\pt}      {\ensuremath{p_{\rm T}}\xspace}
\renewcommand{\pttrue}  {\ensuremath{p_{\rm T}^{\rm true}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}
\newcommand{\NjetStd}   {\ensuremath{N_{\rm jet}^{R4}}\xspace}


% Insitu mass validation
\newcommand{\rtrkjet}       {\ensuremath{r_{\rm track \; jet}}\xspace}
\newcommand{\rtrkjetPt}     {\ensuremath{\rtrkjet^{p_T}}\xspace}
\newcommand{\rtrkjetM}      {\ensuremath{\rtrkjet^{M}}\xspace}
\newcommand{\rtrkjetPtData} {\ensuremath{\rtrkjet^{p_{T},{\rm data}}}\xspace}
\newcommand{\rtrkjetMData}  {\ensuremath{\rtrkjet^{M,{\rm data}}}\xspace}
\newcommand{\rtrkjetPtMC}   {\ensuremath{\rtrkjet^{p_{T},{\rm MC}}}\xspace}
\newcommand{\rtrkjetMMC}    {\ensuremath{\rtrkjet^{M,{\rm MC}}}\xspace}
\newcommand{\RtrkjetPt}     {\ensuremath{R_{r{\rm \; track \; jet}}^{p_T}}\xspace}
\newcommand{\RtrkjetM}      {\ensuremath{R_{r{\rm \; track \; jet}}^{M}}\xspace}

% Jet substructure related
\newcommand{\subjetpt}  {\ensuremath{p_{T}^{\rm subjet}}\xspace}
\newcommand{\yij}       {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}      {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}      {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}       {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}       {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}   {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}   {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\yOneTwo}   {\ensuremath{y_{1}}\xspace}
\newcommand{\yTwoThr}   {\ensuremath{y_{2}}\xspace}
\newcommand{\yOneTwoDef}{\ensuremath{\yOneTwo=\DOneTwo/\mjet}\xspace}
\newcommand{\yTwoThrDef}{\ensuremath{\yTwoThr=\DTwoThr/\mjet}\xspace}
\newcommand{\xj}        {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}   {\ensuremath{J^{(eik),c} (\mjet,\pT,R)}\xspace}
\newcommand{\tauN}      {\ensuremath{\tau_N}\xspace}
\newcommand{\tauTwoOne} {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo} {\ensuremath{\tau_{32}}\xspace}
\newcommand{\dip}       {\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dipOneTwo} {\ensuremath{\dip_{12}}\xspace}
\newcommand{\dipTwoThr} {\ensuremath{\dip_{23}}\xspace}
\newcommand{\dipOneThr} {\ensuremath{\dip_{13}}\xspace}

% Samples
\newcommand{\Zprimett}  {\ensuremath{\Zprime\ra t\bar{t}}\xspace}
\newcommand{\Zqq}       {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}       {\ensuremath{W\ra q\bar{q}}\xspace}


% Random
\newcommand{\mpi}{multiple parton interactions\xspace} % David/Emily using multiple proton interactions.
                                                                                                                 
\newcommand{\SUSY}     {SUSY\xspace}
\newcommand{\Ebar}     {\ensuremath{\bar E}\xspace}
\newcommand{\Dbar}     {\ensuremath{\bar D}\xspace}
\newcommand{\Ubar}     {\ensuremath{\bar U}\xspace}
\newcommand{\rp}       {\ensuremath{R_p}\xspace}
\newcommand{\rpv}      {\ensuremath{\not \!\! R_p}\xspace}
\newcommand{\rpvm}     {\ensuremath{\not  R_p}\xspace}
\newcommand{\Wrp}      {\ensuremath{W_{\rp}}\xspace}
\newcommand{\Wrpv}     {\ensuremath{W_{\rpvm}}\xspace}
\newcommand{\rpmssm}   {\ensuremath{R_p}-MSSM\xspace}
\newcommand{\rpvmssm}  {\ensuremath{\rpv}-MSSM\xspace}
\newcommand{\lam}      {\ensuremath{\lambda}\xspace}
\newcommand{\lamp}     {\ensuremath{\lam^{\prime}}\xspace}
\newcommand{\lampp}    {\ensuremath{\lam^{\prime\prime}}\xspace}
\newcommand{\lamijk}   {\ensuremath{\lambda_{ijk}}\xspace}
\newcommand{\lampijk}  {\ensuremath{\lam_{ijk}^{\prime}}\xspace}
\newcommand{\lamppijk} {\ensuremath{\lam_{ijk}^{\prime\prime}}\xspace}
\newcommand{\msquark}  {\ensuremath{m_{\squark}}\xspace}
\newcommand{\mgluino}  {\ensuremath{m_{\gluino}}\xspace}
\newcommand{\ptgluino} {\ensuremath{\pt^{\gluino}}\xspace}
\newcommand{\ABCD}     {\ensuremath{ABCD}\xspace}
\newcommand{\CLs}      {\ensuremath{{\rm CL}_{s}}\xspace}
\newcommand{\CLb}      {\ensuremath{{\rm CL}_{b}}\xspace}
\newcommand{\CLsb}     {\ensuremath{{\rm CL}_{s+b}}\xspace}


%%% EDITORIAL tools

% Text color
\newcommand{\redtext}[1]      {{\textcolor{red} #1}}
\newcommand{\bluetext}[1]     {{\textcolor{blue} #1}}

% Editorial notes
\newcommand{\editnote}[2][Ed] {{[{\em{\bf\em \textbf{{#1}:} }{\it #2}}]}}

% Placeholder figure with text
\newcommand{\placeholder}[3]  {\framebox[#1]{\begin{minipage}[t]{#1} \vspace{0pt} \centering #3 \vspace{#2}\end{minipage}}}

% Block commenting
\newcommand{\comment}[1]{}

% Horizontal rules
\newcommand{\T}               {\rule{0pt}{2.6ex}}
\newcommand{\B}               {\rule[-1.2ex]{0pt}{0pt}}

% Figure, section, subsection refs
\newcommand{\figref}[1]       {figure~\ref{fig:#1}}
\newcommand{\Figref}[1]       {Figure~\ref{fig:#1}}
\newcommand{\figsref}[2]      {figures~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\Figsref}[2]      {Figures~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figrange}[2]     {figures~\ref{fig:#1}--\ref{fig:#2}}
\newcommand{\eref}[1]         {eq.~\ref{eq:#1}}
\newcommand{\Eref}[1]         {Eq.~\ref{eq:#1}}
\newcommand{\equref}[1]       {eq.~(\ref{eq:#1})}
\newcommand{\Equref}[1]       {Eq.~(\ref{eq:#1})}
\newcommand{\tabref}[1]       {table~\ref{tab:#1}}
\newcommand{\Tabref}[1]       {Table~\ref{tab:#1}}
\newcommand{\secref}[1]       {section~\ref{sec:#1}}
\newcommand{\Secref}[1]       {Section~\ref{sec:#1}}
\newcommand{\appref}[1]       {appendix~\ref{app:#1}}
\newcommand{\bibref}[1]       {\cite{#1}}

% Other symbols
\newcommand{\lsim}            {{\stackrel{<}{\sim}}}

